Foreground-Covering Prototype Generation and Matching for SAM-Aided Few-Shot Segmentation

We propose Foreground-Covering Prototype Generation and Matching to resolve Few-Shot Segmentation (FSS), which aims to segment target regions in unlabeled query images based on labeled support images. Unlike previous research, which typically estimates target regions in the query using support prototypes and query pixels, we utilize the relationship between support and query prototypes. To achieve this, we utilize two complementary features: SAM Image Encoder features for pixel aggregation and ResNet features for class consistency. Specifically, we construct support and query prototypes with SAM features and distinguish query prototypes of target regions based on ResNet features. For the query prototype construction, we begin by roughly guiding foreground regions within SAM features using the conventional pseudo-mask, then employ iterative cross-attention to aggregate foreground features into learnable tokens. Here, we discover that the cross-attention weights can effectively alternate the conventional pseudo-mask. Therefore, we use the attention-based pseudo-mask to guide ResNet features to focus on the foreground, then infuse the guided ResNet feature into the learnable tokens to generate class-consistent query prototypes. The generation of the support prototype is conducted symmetrically to that of the query one, with the pseudo-mask replaced by the ground-truth mask. Finally, we compare these query prototypes with support ones to generate prompts, which subsequently produce object masks through the SAM Mask Decoder. Our state-of-the-art performances on various datasets validate the effectiveness of the proposed method for FSS. Our official code is available at https://github.com/SuhoPark0706/FCP

==> figure/figure1.tex <==
\begin{figure}[t!]
    {\includegraphics[width=0.47\textwidth]{figure/figure1_v13.pdf}}
    \centering
    \caption{
    %%%%%%%%%%%%%%%% v1 %%%%%%%%%%%%%%%%%%%
    % Comparison between VRP-SAM and Ours.
    % (a) We show the IoU between the query foreground and the attention map from support prototypes to the query. 
    % Compared to VPR-SAM, our method produces a high-quality attention map, focusing on the foreground.
    % (b) We compare the na\"ive and attention-based pseudo masks used to facilitate classification in VRP-SAM and our method, respectively.  
    % The visualizations and the IoU distribution with query foreground confirm the effectiveness of our attention-based pseudo-mask.
    %%%%%%%%%%%%%%%% v2 %%%%%%%%%%%%%%%%%%%
    % (a) We measure the IoU between the query foreground and the attention map from support prototypes to query features. Our method produces a higher-quality attention map, more accurately focusing on the query foreground.
    % benefiting from the construction of query prototypes whereas VRP-SAM relies on direct relations to query pixels.
    % Both qualitative result and quantitative (IoU distribution with query foreground) results confirm the effectiveness of our attention-based pseudo-mask.
    % (b) We compare the na\"ive pseudo masks proposed by VRP-SAM with our attention-based pseudo mask. The visualizations and the IoU distribution with query foreground confirm that our approach is more fine-grained and reliable.
    %%%%%%%%%%%%%%%% v3 %%%%%%%%%%%%%%%%%%%
    % \SH{
    % Comparison between VRP-SAM and Ours.
    % (a) To show the effectiveness of prototype-to-prototype matching, we show the similarity within the query foreground from prototypes-to-pixels (VRPSAM) and prototypes-to-prototypes (ours).
    % Compared to VPR-SAM, our method achieves higher similarity within the query foregrounds.
    % (b) We compare the na\"ive and attention-based pseudo masks used to approximate foregrounds in VRP-SAM and our method, respectively.  
    % The visualizations and the IoU distribution with query foreground confirm the effectiveness of our attention-based pseudo-mask.}
    %%%%%%%%%%%%%%%% v4 %%%%%%%%%%%%%%%%%%%
    Comparison between VRP-SAM and Ours. \textbf{(a)}~(left) We visualize pixel-wise attention maps of query image compared to support prototype. (right) Summing the scores corresponding to the foreground, our prototype-to-prototype matching achieves a higher average score than prototype-to-pixel matching~(VRP-SAM). \textbf{(b)} We compare the conventional and attention-based pseudo masks generated by VRP-SAM and our method. The visualizations and IoU distribution with query foreground validate the effectiveness of our attention-based pseudo-mask.
    }
\label{fig:fig_1}
\end{figure}

==> figure/figure2.tex <==
\begin{figure}[t!]
    {\includegraphics[width=0.48\textwidth]{figure/figure2_v3.pdf}}
    \centering
    \caption{
    % Comparison between ResNet and SAM Encoder, demonstrating their complementary strengths.
    % % v1
    % % (a) We measure the difference between FG (foreground)-to-FG similarity and FG-to-BG (background) similarity within an image. The higher similarity difference in SAM Encoder shows its superior pixel-level aggregation for prototype construction. 
    % % (b) We measure the difference of similarity between images of the same class (intra-class) and images of different classes (inter-class). The higher similarity difference shown in ResNet indicates that its features are more consistent and robust for feature matching across different images.
    % % v2: similarity 계산 자세한 과정 추가
    % % (a) We calculate the self-cosine similarity map and measure the difference between foreground-to-foreground and foreground-to-background similarities.
    % % (a) Difference between FG-to-FG and FG-to-BG similarities computed through self-cosine similarity map.
    % % \HS{(a)~Difference in cosine similarity between FG-to-FG and FG-to-BG within the image.}
    % (a) Similarity difference between FG-to-FG and FG-to-BG within the image.
    % % The histogram shows the distribution of these differences per image. 
    % % As shown in the histogram, 
    % The higher similarity difference shown in SAM Encoder reflects its superior pixel-level aggregation for prototype construction.
    % % \HS{(a) The histogram visualizes the distribution of similarity differences computed for each image. Compared to ResNet, SAM Encoder shows its superior pixel-level aggregation for prototype construction.}
    % % (b) We compute the average foreground-to-foreground cosine similarity  
    % (b) Difference between the average FG-to-FG similarity
    % %  between an image and another image 
    % of images from the same class (intra-class) or different classes (inter-class). 
    % % The histogram shows the distribution of differences between these similarities for each image. 
    % % The histogram shows ResNet's higher similarity difference, indicating its features are more consistent across different images.
    % Compared to SAM Encoder, ResNet conveys better class consistency across different images.
    Comparison between ResNet and SAM Image Encoder features on 1000 PASCAL VOC images in test dataset, demonstrating their complementary strengths.
    \textbf{(a)} Similarity difference between FG-to-FG and FG-to-BG within the image.
    The higher similarity difference shown in SAM Image Encoder features reflects its superior pixel-level aggregation for prototype construction.
    \textbf{(b)} Difference between the FG-to-FG similarity from the same class (intra-class) and different classes (inter-class).
    Compared to SAM features, ResNet features convey better class consistency across different images.
    }
\label{fig:fig_2}
\end{figure}

==> figure/figure3.tex <==
\begin{figure*}[t]
    \centering
    {\includegraphics[width=0.98\textwidth]{figure/figure3_v12.pdf} }
    \caption{ 
    Overall procedure of Foreground-Covering Prototype Generation and Matching.
    Given the SAM Image Encoder features $G$, we start by guiding the foreground features using the ground-truth mask for the support $M^S$ and a conventional pseudo-mask for the query $M^\text{pseudo}$, then gather these guided features $\bar{G}$ into learnable tokens $P$ through iterative cross-attention.
    However, SAM features lack class consistency across different images, making it challenging to directly construct prototypes. 
    To address this, we utilize ResNet features $F$ to infuse class-consistent properties into the tokens. 
    % \HS{Before applying these properties, we further assist the classification}
    We first guide the ResNet features to enhance the foreground-specific information with the ground-truth mask of the support and an attention-based pseudo-mask for the query $M^{\text{attn}}_{T-1}$.
    The attention-based pseudo-mask, benefiting from SAM's high aggregation capability, provides better precision compared to the conventional pseudo-mask, as shown in the upper right. 
    By infusing the class consistency of the guided ResNet features $\bar{F}$ into the learnable prompts, we obtain both support and query prototypes ($P^S_T$ and $P^Q_T$). 
    As a result, the visual reference prompts are generated by matching the query prototypes with the support ones and these prompts are passed to the SAM Decoder to predict a query mask $M^{\text{pred}}$.
    }
\label{fig:fig_3}
\end{figure*}

% 1 - aggregation guidance 
% 2 - classification guidance

% a - ag & cg 같은 weight

==> figure/figure4.tex <==
\begin{figure}[t!]
    {\includegraphics[width=0.47\textwidth]{figure/figure4_v4.pdf}}
    \centering
    \caption{
    % Qualitative comparison results of Ours and VRP-SAM on the PASCAL-5$^i$ dataset. Naive and Attention-based refer to the na\"ive pseudo mask of VRP-SAM and our attention-based pseudo mask, respectively.
    Qualitative comparison results of Ours and VRP-SAM on the PASCAL-5$^i$ dataset. Conventional and APM refer to the conventional pseudo-mask of VRP-SAM and our Attention-based Pseudo-Mask, respectively.
    }
\label{fig:fig_4}
\end{figure}

==> figure/num_layer.tex <==
\begin{figure}[t!]
    {\includegraphics[width=0.47\textwidth]{figure/figure5_v2.pdf}}
    \centering
    \caption{
    Ablation study for varying the number of aggregation steps for prototype construction. Prediction and APM denote our model's query mask prediction and Attention-based Pseudo Mask, respectively.
    }
\label{fig:num_layers}
\end{figure}
